From Adoption to Deployment: A Qualitative Study on AI Integration in Software Development Practice

The increasing adoption of Large Language Models (LLMs) as AI components in modern software systems introduces distinct security risks to the software supply chain. While many considerations and safety mechanisms are in place for components of the traditional software supply chain, the recent rapid adoption of AI components and platforms has overlooked these hard learned lessons. Selecting and integrating AI models without clear guidance on how these choices affect system security may leave applications vulnerable to threats, such as malicious components, data leakage, and unintended behavior. The goal of this study is to understand practitioners' decision making process and security considerations in selecting and integrating AI components through an exploratory semi-structured interview study. Toward this goal, we conducted semistructured interviews with 22 software developers, architects, and AI practitioners across diverse organizations about how they integrate AI components into their software. Our analysis finds that practitioners' model selection is predominantly driven by functional criteria, including performance, accuracy, cost, and specific features, e.g., tool calling or multimodal support, while security is rarely considered as an evaluation criterion. We observe a consistent lack of security concern throughout the AI component integration process, with established software supply chain lessons overlooked or ignored. The industry is repeating the historically costly mistakes of early software dependency management, prioritizing rapid reuse and availability over security and provenance. We distill our findings into actionable recommendations for AI adopters, model providers, and researchers, advocating for a proactive, security-by-design approach that integrates security evaluation into component selection and sustains it throughout the software development lifecycle.

==> sections/00a-glossary.tex <==
%--------------------------
% PACKAGES
%--------------------------
% Add any additional packages here

\usepackage[utf8]{inputenc} % should not be necessary with current LaTeX versions
\usepackage[T1]{fontenc}

% Colors (mainly used for comments or tikzfigures)
\usepackage[dvipsnames,table]{xcolor}
% This occasionally breaks, if it does comment out xcolor in the template your using or here
% \usepackage{xcolor-material} % more colors according to material design guidelines

% Encoding and text options
\usepackage[normalem]{ulem}
\usepackage{fontawesome}
\usepackage{csquotes}
\usepackage{setspace}

% Figures and graphics
\usepackage{svg}
\usepackage{graphicx}
\usepackage{graphics}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{float}
\usepackage{tcolorbox}

% TikZ (load once with all libraries)
\usepackage{tikz}
\usetikzlibrary{shapes,arrows,fit,matrix,positioning,decorations.pathreplacing,arrows.meta}

% Fonts
\usepackage{times}
\usepackage[gen]{eurosym}

% Hyperref MUST come before hyperxmp
\usepackage{hyperref}
\usepackage{hyperxmp}

% Tables
\usepackage{tabularx}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage[para, flushleft]{threeparttable}
\usepackage{array}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{tablefootnote}
% \usepackage{urlref}

% Fix some weird behavior when using colored rows within tabularx. see https://tex.stackexchange.com/questions/297345/why-is-the-start-row-of-rowcolors-ignored-in-tabularx/297357
\newcounter{tblerows}
\expandafter\let\csname c@tblerows\endcsname\rownum

% Lists
\usepackage{enumitem}

% Utility packages
\usepackage{etoolbox}

%\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}} % left fixed width
%\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}} % center fixed width
%\newcolumntype{R}[1]{>%{\raggedleft\arraybackslash}p{#1}} % flush right fixed width

\newcolumntype{R}[2]{%
    >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
    l%
    <{\egroup}%
}
\newcommand*\rot{\multicolumn{1}{R{45}{1em}}}% no optional argument here, please!

%--------------------
% REFERENCES
%--------------------

% Better display of citation URLs
\usepackage{xurl}
\PassOptionsToPackage{hyphens,spaces,obeyspaces}{xurl}

% IMPORTANT: Make sure natbib is NOT loaded anywhere
% Check your document class (\documentclass{}) - some templates load natbib automatically
% If your document class loads natbib, you may need to use a different class or disable it
% Uncomment the line below ONLY if your document class loads natbib:
% \let\bibhang\relax
% \let\citename\relax

\usepackage[backend=biber]{biblatex}
\addbibresource{ref.bib}

% Custom cite command for full name
\DeclareCiteCommand{\citeauthorfull}
    {\boolfalse{citetracker}%
    \boolfalse{pagetracker}%
    \DeclareNameAlias{labelname}{given-family}%
    \usebibmacro{prenote}}
    {\ifciteindex
        {\indexnames{labelname}}
        {}%
        \printnames{labelname}}
        {\multicitedelim}
{\usebibmacro{postnote}}

%--------------------
% Authors related information
%--------------------

% ORCID IDs of teamusec group members
\usepackage{orcidlink}
\newcommand{\orcidSascha}{\orcidlink{0000-0002-5644-3316}}
\newcommand{\orcidAlex}{\orcidlink{TBD}}
\newcommand{\orcidDominik}{\orcidlink{TBD}}
\newcommand{\orcidHarjot}{\orcidlink{TBD}}
\newcommand{\orcidJan}{\orcidlink{0000-0002-6994-7206}}
\newcommand{\orcidJuliane}{\orcidlink{TBD}}
\newcommand{\orcidNico}{\orcidlink{TBD}}
\newcommand{\orcidNiklas}{\orcidlink{0000-0001-5621-8461}}
\newcommand{\orcidNoah}{\orcidlink{TBD}}
\newcommand{\orcidPhilip}{\orcidlink{TBD}}
\newcommand{\orcidSabrina}{\orcidlink{TBD}}
\newcommand{\orcidSandra}{\orcidlink{TBD}}

% Email addresses of teamusec group members

%--------------------
% DOCUMENT SPECIFIC SETTINGS
%--------------------
% Document specific settings such as hyphenation rules and custom text macros go here

% Hypenation
%\hyphenation{Whats-App}  % add custom hyphenations like this

% Macros
\newcommand{\ie}{i.\,e.}
\newcommand{\eg}{e.\,g.}
\newcommand{\Eg}{E.\,g.}
\newcommand{\cf}{cf.}
\newcommand{\perc}{\,\%}
% \newcommand{\mail}{e-mail} % add custom shortcuts like this

% custom environment for the research questions in the introduction
% needs work!
\newenvironment{rqs}
{\begin{description}}
{\end{description}}

% custom environment for the contributions in the introduction
% needs work!
%\newenvironment{contrib}
%{\begin{description}}
%{\end{description}}

%Table extra
\newcommand{\MarkX}{ \tikz\draw[black,fill=black] (0,0) circle (.5ex); }

% Quote formatting
\AtBeginEnvironment{quote}{\vspace{-0.9em}}
\AtEndEnvironment{quote}{\vspace{-0.5em}}
\newcommand{\quotedev}[2]{%
\begin{quote}
\color{Orchid}
\emph{\enquote{#1}}~{[#2]}
\end{quote}
}
\newcommand{\participantQuote}[2]{{\color{Orchid}\textit{``#1''}~({#2})}}

